Differentially Private Query Release Through Adaptive Projection

We propose, implement, and evaluate a new algorithm for releasing answers to very large numbers of statistical queries like $k$-way marginals, subject to differential privacy. Our algorithm makes adaptive use of a continuous relaxation of the Projection Mechanism, which answers queries on the private dataset using simple perturbation, and then attempts to find the synthetic dataset that most closely matches the noisy answers. We use a continuous relaxation of the synthetic dataset domain which makes the projection loss differentiable, and allows us to use efficient ML optimization techniques and tooling. Rather than answering all queries up front, we make judicious use of our privacy budget by iteratively and adaptively finding queries for which our (relaxed) synthetic data has high error, and then repeating the projection. We perform extensive experimental evaluations across a range of parameters and datasets, and find that our method outperforms existing algorithms in many cases, especially when the privacy budget is small or the query class is large.

==> addl_exps.tex <==
\subsection{Additional Experiments}
Some measures we could consider: 
\begin{itemize}
    \item Wasserstein loss (approximated with second discriminator) in-sample and out-of-sample
    \item Inception score (for image data only?)
    \item JS distance
    \item For Gaussians, measure KDE error?
    \item Success on downstream prediction tasks
\end{itemize}

It seems like empirical (Wasserstein, JS) loss is often measured with respect to the training data, but I think we should focus on out of sample performance. An interesting result would be if privacy actually helps with generalization.

Worth looking further into metrics discussed here: \cite{arora2017generalization}. One point this paper makes is that polynomial samples won't well-approximate the true distribution w.r.t\ JS or Wasserstein distance, and as such they argue that these are poor generalization measures. I somewhat disagree ---  I think a more natural benchmark would be to consider e.g.\ Wasserstein distance with respect to a second sample of the same size, permitting more of an apples to apples comparison. If it hasn't been done already, it seems possible to prove generalization bounds for Wasserstein distance when training privately with respect to a second sample of the same size. \wb{Upon closer inspection, their point is a little more subtle --- the class of 1-Lipschitz functions is too large to apply uniform convergence, }

Batch normalization?

\wb{LFW, IDC (used in \cite{wu2019generalization}) ?}


Use ``standard architectures'' for each dataset to start, then evaluate on random architectures as a stretch goal (there's gotta be starter code out there for doing this).
We consider both weight clipping and gradient penalties as regularization methods for enforcing the Lipschitz constraint on the discriminator required by the Wasserstein distance.



\subsection{Evaluating synthetic data quality}

For each dataset, but beginning with the simplest ones: 
\begin{itemize}
    \item Evaluate each descent method (measure: Wasserstein loss using second discriminator, trained after termination on final model, using $N$ fake samples, against $N$ test points)
    \item Holding $\epsilon$, $\delta$, and minibatch size fixed, vary number of steps vs noise amount (for both 1:1 and 5:1)
\end{itemize}


\subsection{Membership detection attacks}

Show the extent to which membership attacks succeed

Ideally, we should show that generated points are often very close to training data points even when training with optimism. Seems like there are sensible handcrafted measures we could use, such as quantiles for norm distance to closest point. Will also dig around to see if there are any standards for this task. 




\subsection{Limit cycles when training GANs with DP-SGD}


If we're seeing good initial results with optimistic methods, we could try to recreate the experiments from \cite{daskalakis2017training} which show a sharp distinction between OMD and GD for convergence on simple distributions. Will do more lit review on the limit cycles problem, would be good to understand how this is ``observed'' in practice. What are the standard approaches for choosing when to sample, if training doesn't converge? 

Can we simultaneously avoid membership detection issues while improving stability of training with POMD?

==> conclusion.tex <==
\section{Conclusion}
In this work, we proposed a novel approach DCO for synhtetic data generation with privacy guarantees. We used both Zero-Sum and $\ell_{infty}$-norm as and objective and showed that the Zero-Sum DCO performs better than $\ell_{infty}$-norm DCO. We also provided a holistic view of GAN-based approaches. Our results show that simple Zero-Sum DCO approach performs as well as GAN-based approaches for linearly separable datasets. However, GAN-based approaches perform better to learn more complex representations.


==> experiments.tex <==
\section{Experiments}



\subsection{Experimental Setup}

\paragraph{Datasets.} We conduct experiments on a number of synthetic datasets --- a grid of Gaussians, intersecting crescents, nested circles, and imbalanced blobs --- as well as several image and tabular datasets, including MNIST, CIFAR-10, and the Breast Cancer, Forest Fires, Blog Feedback, and Adult Income datasets from the UCI Machine Learning Repository \cite{Dua:2019}. For tabular datasets, we restrict to numerical or binary columns.
We also conduct experiments with the image datasets MNIST and CIFAR-10.
\wb{KK: add citations}


\paragraph{Model architectures.}
For each of the
%tabular (including toy) 
datasets, we use standard feedforward networks with ReLU activation, with 6 layers for the generator and 8 for the discriminator, all of width 512, and an input space of 256 dimensions for the generator. We use the Wasserstein distance with gradient penalty as our loss function.
%For image datasets, we use... \wb{testing a few options still}
%For the Census, image and other tabular data experiments, we will use the same architecture and training regime as in \cite{tantipongpipat2019differentially}. Initially training an autoencoder privately to learn how to map the data into a latent space of lower dimensionality. Once the autoencoder is trained, the generator is trained to transform an input gaussian distribution into the latent space which is then transformed by the decoder into the space of the original data. The discriminator is trained privately. For a diagram, refer to \ref{architecture}.

\paragraph{Evaluation benchmarks.} For toy datasets, we evaluate quality by estimating the Wasserstein distance between the learned and target distributions using a second discriminator network (trained non-privately with Adam, using the same architecture), as well as through manual inspection of samples. \wb{KK: Can we not directly measure the distance by generating the same number of synthetic data points as the original ones?}\wb{I don't believe computing Wasserstein/optimal transport is poly-time tractable for arbitrary domains even with fixed sample sizes, as it requires taking a maximum over all 1-Lipschitz functions, or a minimum over all joint distributions with the correct marginals.} Additionally, for real datasets we evaluate quality by measuring the performance of machine learning models trained on generated data.


\paragraph{Model selection.} For the Wasserstein and prediction objectives, we take the maximum over models saved periodically over training. For visualizing samples from toy datasets we use the final model.
\iffalse
Which model or combination of models should be used for generating synthetic data? For initial experiments we have simply used the final model \wb{KK: what does this mean?}, but additional selection methods may be useful in improving performance for a given privacy budget, such as:
\begin{itemize}
    \item Choosing the best model for the evaluation metric using private selection. An example being \cite{jingcheng2019PrivateSelection} which allows for model choice without too much additional loss in privacy
    \item Using the historical distribution over models (this is "theoretically correct" in linear games, and mixtures have generalization benefits \cite{arora2017generalization}) 
    \item Averaging the parameters of learned models (often used in practice, see e.g. \cite{yazc2018unusual})
    \item Post-GAN Boosting \cite{neunhoeffer2020private}
\end{itemize}
We intend to explore these with further experimentation.
\fi

\paragraph{Parameters affecting privacy.}

The privacy loss $\epsilon$ is computed as a function of
the number of training samples ($N$),
the number of discriminator minibatch steps,
    %(1:1 and 5:1 ratio used in \cite{daskalakis2017training})
minibatch and microbatch sizes,
the amount of noise added to gradient estimates,
and the target additive privacy loss $\delta$.
The scale of noise is governed by a multiplier $\sigma$ as well as the gradient clipping bound $C$. The privacy loss does not depend on $C$, but calibrating it correctly is important as it results in excessive noise if it is too large and damages gradients if too small. As such, for a fixed dataset and target privacy loss, we have a number of degrees of freedom in satisfying the privacy guarantee.
Understanding this calibration process is a major goal of our work.
%ow does performance change as we vary epsilon? Increase training times?
%It may be natural to think of $N$ and $\delta$ as fixed ($\delta = 1 / N$?), and so for a fixed privacy level $(\epsilon = 1?)$ we have three degrees of freedom in achieving the budget. We could also consider varying the noise level over the course of training. \wb{Break into segments, compute privacy loss individually, and sum? Or are there stronger adaptive composition theorems?}

\paragraph{Implementation.}
We train our networks with PyTorch, using the Pyvacy library \cite{Waites2019PyVacyTP} for privacy enforcement. Pyvacy handles the batching of the dataset into mini- and microbatches, gradient manipulation and privacy accounting. The authors implemented the optimistic versions of SGD and Adam.

\subsection{\wb{Experiment: }Visualizing Toy Data}

Training on \textasciitilde 1M points, we are able to achieve reasonable-looking synthetic data using Optimistic Adam, with values of $\epsilon$ ranging from \textasciitilde 2500-5000, shown in \Cref{fig:toydata}. This is, admittedly, a very high $\epsilon$, yet it can be improved by adjusting the L2 clipping norm of the gradients to the median of gradients in non-private training. These toy datasets are also \textit{hard}, non-Gaussian datasets. Results are comparable with Adam and worse with other optimizers. Here, dots denote the "real data" and pluses denote the synthetic data, where color is a feature. For the grid of Gaussians, we display the kernel density estimation for synthetic data. \wb{KK: Will be helpful to state the parameters involved, e.g., mean/variance values}

\begin{figure}
    \centering
    \includegraphics[width=5.5cm]{figs/1048577_OptAdam_privTrue_i30001_mb64_n0.05_7-29-2020_4_9train.png}
    \includegraphics[width=5.5cm]{figs/1048577_OptAdam_privTrue_i40001_mb64_n0.05_7-29-2020_0_6train.png}
    \includegraphics[width=5.5cm]{figs/1048576_OptAdam_privTrue_i50001_mb64_n0.04_7-29-2020_5_27train.png}
    \includegraphics[width=5.5cm]{figs/1048577_OptAdam_privTrue_i50001_mb64_n0.04_7-29-2020_4_55train.png}
    \caption{Private GANs Trained on Toy Data}
    \label{fig:toydata}
\end{figure}

\subsection{\wb{Experiment: }Choosing the Best Optimizer for GANs}
In \Cref{fig:wloss}, we show the progress of several training algorithms over time on Gaussian grid toy data, for varying levels of the noise parameter $\sigma$ for gradient estimates, evaluating by periodically computing the Wasserstein distance for the network. Performance degrades as noise increases, resulting in more iterations before convergence, and training fails to converge for all optimizers for $\sigma = 0.1$. Adam, Optimistic Adam, and RMSprop perform comparably well across noise levels, whereas Adagrad fails to converge in each instance. For the latter three optimizers we evaluate different ratios for discriminator and generator steps, and find that a ratio of 5, particularly for Adam, consistently results in better performance.

\begin{figure}
    \centering
    \includegraphics[width=5.5cm]{figs/many_opts_001.png}
    \includegraphics[width=5.5cm]{figs/many_opts_003.png}
    \includegraphics[width=5.5cm]{figs/many_opts_05.png}
    \includegraphics[width=5.5cm]{figs/many_opts_0.1.png}
    \includegraphics[width=5.5cm]{figs/BESTOPT4_gaussiangrid_0.1.png}
    \includegraphics[width=5.5cm]{figs/BESTOPT4_gaussiangrid_0.05.png}
    \includegraphics[width=5.5cm]{figs/BESTOPT4_gaussiangrid_0.01.png}
    \caption{Wasserstein Loss across Optimizers and Noise Levels}
    \label{fig:wloss}
\end{figure}
\wb{
\paragraph{Proposal.} For the Gaussian Grid, MNIST, and Breast Cancer datasets, we plot the estimated Wasserstein loss over training, for $\sigma \in \{0.01, 0.05, 0.1\}$, using the Adam, OptAdam, and RMSProp optimizers, both for G-D ratios 1 and 5 (9 plots total).
}
\subsection{\wb{Experiment: }GANs for Downstream ML}

%\paragraph{Proposal.} 
In addition to evaluating with Wasserstein loss, another useful metric is understanding the usefulness of synthetic data for machine learning.
Using Adam with a ratio of 5, for the Crescents, Breast Cancer, and Adult datasets, we
 we generate synthetic data using GANs, which we then use to train a set of classification models, whose performance we evaluate on the original data.
For each dataset, we train a GAN for 25K iterations using $\sigma \in \{0.01, 0.05, 0.1, 0.5, 1.5 \}$.
For each $\sigma$, we train using all clipping parameters $C \in \{0.2, 0.5, 1, 2.5\}$.
%For determining clipping parameters, we conduct non-private training and compute percentiles of the gradient norms over training ($\{30, 50, 70, 90\}$) and repeat the experiment for each clipping parameter (as well as for  $C \in \{0.1, 1\}$).
For any fixed $\epsilon$ and $\sigma$, there is some prefix of the sequence of 25K iterations for which the privacy budget is not exhausted. 
For each $\epsilon$, we select the best result by searching over $\sigma$, $C$, and the corresponding prefix sequence. 
The (best) performance of several classifiers, for both accuracy and F1 score, is plotted as a function of $\epsilon$ and displayed in \Cref{fig:gan_best_ml_eps}.
Results for some fixed parameter settings, benchmarked with the performance of classifiers trained directly on the data, are shown in \Cref{fig:gan-classification}.


\begin{figure}
    \centering
    \includegraphics[width=5.5cm]{figs/cancer_eps_best_ML_2.png}
    \includegraphics[width=5.5cm]{figs/crescents_eps_best_ML_3.png}
    \includegraphics[width=5.5cm]{figs/adult_eps_best_ML_3.png}
    \caption{GAN Classification Evaluations vs $\epsilon$ (Cancer, Crescents, Adult)}
    \label{fig:gan_best_ml_eps}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=5.5cm]{figs/test_MLplotPRIV10e6.png}
    \includegraphics[width=5.5cm]{figs/test_MLplotPRIV10e8.png}
    \includegraphics[width=5.5cm]{figs/test_MLplotPRIV10e14.png}
    \includegraphics[width=5.5cm]{figs/test_MLplot_NONPRIV.png}
    \caption{Classification using Synthetic Data from GANs ($\epsilon = [10^6, 10^8, 10^{14}, \infty]$)}
    \label{fig:gan-classification}
\end{figure}

The results demonstrate that the utility of the synthetic data increases as the privacy parameter $\epsilon$ (low privacy) increases as expected due to privacy and utility trade-off.


\subsection{\wb{Experiment: }Direct Consistency Optimization for Downstream ML}
We also evaluate the usefulness of synthetic data generated by direct consistency optimization, computed both using the zero-sum game approach and gradient descent on the $\ell_{\infty}$ norm. 
As we did for GANs, results for increasing $\epsilon$ are shown in \Cref{fig:zs_dco_best_ml_eps} and \Cref{fig:linf_dco_best_ml_eps}, for the zero-sum game and $\ell_{\infty}$ optimization methods, respectively. Fixed-parameter comparisons to non-private training are shown in \Cref{fig:dco-classification}. In the appendix, we visualize the generated synthetic Crescents data for each method (in \Cref{fig:dco-crescents}).

 Results in \Cref{fig:zs_dco_best_ml_eps} show that the utility of the synthetic data increases as the parameter $\epsilon$ increases for both datasets when Zero-Sum DCO is used. However,  $\ell_{\infty}$-norm DCO performs poorly for both datasets.

\begin{figure}
    \centering
    \includegraphics[width=5.5cm]{figs/cancer_eps_best_ML_ALL_game.png}
    \includegraphics[width=5.5cm]{figs/crescents_eps_best_ML_ALL_game.png}
    \caption{Zero-Sum DCO Classification Evaluations vs $\epsilon$ (Cancer, Crescents)}
    \label{fig:zs_dco_best_ml_eps}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=5.5cm]{figs/cancer_eps_best_ML_ALL_opt.png}
    \includegraphics[width=5.5cm]{figs/crescents_eps_best_ML_ALL_opt.png}
    \caption{$\ell_{\infty}$-norm DCO Classification Evaluations vs $\epsilon$ (Cancer, Crescents)}
    \label{fig:linf_dco_best_ml_eps}
\end{figure}

\begin{figure}
    \centering
    \includegraphics[width=5.5cm]{figs/ML_evals_game.png}
    \includegraphics[width=5.5cm]{figs/ML_evals_opt.png}
    \caption{Classification using Synthetic Data from DCO (Zero-Sum and $\ell_{\infty}$-norm, $\epsilon = 1000$)}
    \label{fig:dco-classification}
\end{figure}

\wb{
We can do this concurrently with the previous experiment. Plot organization will be equivalent, except factored by $\sigma$, as we are computing several losses for each. One question to explore will be the extent to which success across the two metrics is correlated.
}



%\paragraph{Proposal:} Run both the Game Theory (with varying $\eta$) and $\ell_{\infty}$ variants of the procedure, for varying values of $\epsilon$, on each dataset. Test the performance using the same evaluations as in \Cref{sec:gan-ML-exp}.


%\paragraph{Prediction:} The circles and crescents datasets will be hard/impossible to classify with this approach. Regression and classification may be somewhat successful (better than random) on tabular datasets.

\subsection{GANs vs DCO}
On the whole, we find that GANs are often capable of generating data which is useful for classification subject to some degree of differential privacy. A barrier to strong results for the Cancer dataset is that we train on only $2^9$ points, which requires adding substantial noise for maintaining privacy. Here, DCO reaches almost 80\% accuracy at $\epsilon=8$, whereas this is not attained until $\epsilon=64$ for GANs.
For the Crescents dataset (which has balanced labels) with $2^{15}$ points, we are able to obtain results above 80\% even at $\epsilon=1$ and can approach perfect classification as $\epsilon$ increases.
DCO does not result in nearly as high levels of accuracy even for large $\epsilon$, but the generated data can be sufficient for approximating the performance of the best non-private {\it linear} model at smaller values of $\epsilon$. The crescents example is particularly telling, as labels are separable by a low-degree polynomial but not by a linear classifier.
Holistically, we find that when there is enough data, GANs are more powerful for creating synthetic datasets which preserve more complex structures (non-Gaussian features, non-linear feature relationships) in datasets. However, if data is limited and linear models are appropriate for the classification task, DCO can create data preserving these relationships at a modest privacy cost. 


%\paragraph{Prediction:} GANs will perform well on average but not worst-case inner product/correlation, and direct consistency optimization will perform poorly on Wasserstein distance

==> old.tex <==

\iffalse
Many organizations face the challenge of finding ways to make use of sensitive data.
Datasets containing sensitive information are held by many individual teams, who cannot share datasets at will for fear of compromising the information. 
Further, even if analysis can be conducted by trustworthy parties, the public outputs of these analyses can compromise the privacy of records in the dataset.
Healthcare and finance are prominent domains where these challenges arise frequently. Practical data science workflows in these areas often demand unfettered access to a dataset; a desirable solution would be the ability to create a {\it synthetic} dataset which is statistically similar to the original, and useful for analysis, yet protects the privacy of individual records. Refer to Table 1 in \cite{tantipongpipat2019differentially} for a survey of differentially private synthetic data generation methods.
{ In this paper, we empirically evaluate the success of two families of techniues for synthetic data generation: {\it differentially private GANs} and {\it direct consistency optimization} for families of queries.}

{\it Generative adversarial networks} or GANs were first introduced in \cite{goodfellow2014generative}. They have provided an avenue to generate rich synthetic data in high dimensional spaces. Goodfellow et al. created a zero sum game played by two neural networks, a Generator and a Discriminator. Where the former learns a function to transform an input distribution into the distribution that training points are sampled from. The Generator is rewarded for creating points that the Discriminator cannot distinguish as real or fake and the Discriminator is rewarded for correctly distinguishing synthetic points and real points. GANs have seen success in generating convincing human faces \cite{karras2019analyzing}, colorizing video \cite{jantic2020deoldify} and generating synthetic datasets \cite{choi2017generating, Park_2018, xu2019modeling}.

{\it Differential privacy} has emerged as a gold standard for privacy-preserving data analysis. When satisfied by an algorithm, it provably prevents membership attacks even with auxiliary information, and is robust to postprocessing. Additionally, the quantified privacy guarantee degrades gracefully under composition \cite{privacybook}.
Differentially private mechanisms often restrict access to the dataset to a pre-specified class of queries, which can be insufficient for typical analysis procedures.
Creating a synthetic dataset which approximately preserves answers to a large class of queries is possible from an information-theoretic perspective, and would mitigate the restrictions of interactive mechanisms, but this is computationally intractable in general.
Oracle-efficient approaches are presented in \cite{neel2018use} and \cite{Vietri2019NewOA}, which bear some similarity to the training procedure for GANs.
One solution is to forgo the goal of provably preserving a class of queries in lieu of other metrics of closeness or usefulness.
Examples are distributional distances such as those in training GANs, as well as the success of machine learning models trained on synthetic data when evaluated on the original distribution. 


GANs trained subject to differential privacy are a leading candidate for practical solutions to private synthetic data generation. Private GANs were introduced in were \cite{xie2018differentially}, and several other variants have since been proposed; see \cite{dpgansurvey} for an overview. 
In particular, GANs have been studied as a tool for privately generating synthetic data for use in downstream inference tasks including computer vision and healthcare applications \c.


Nearly all of these variants obtain their privacy guarantees by training networks with differentially private SGD
(as introduced in \cite{Abadi_2016}), 
and often use Wasserstein GAN architectures (from \cite{arjovsky2017wasserstein}). We focus on WGANs but consider a larger set of training algorithms.
GANs do not always converge in practice, and are vulnerable to issues such as mode collapse and suboptimal equilibria; avoiding these issues can require delicate hyperparameter tuning.
When privacy is not a concern, the only barrier to hyperparameter tuning is computational, as one can search over the hyperparameter space and conduct an entire training cycle to evaluate each setting. However, this contributes to privacy loss, which must accounted for, and would substantially degrade the privacy guarantees from a single training cycle. Papers on private GANs typically do not conduct hyperparameter search, relying on baselines from prior work, and we believe this may be a contributing factor to the performance gap between private and non-private GANs. There is the additional challenge of selecting parameters for enforcing privacy, such as the tradeoff between gradient clipping, noise levels, and training time in achieving a privacy target.
This motivates the question which we aim to address in this paper:
{\it how can we get the most mileage out of our privacy budget when generating synthetic data?}\\

Our contributions are as follows:
\begin{itemize}
    \item We provide a comprehensive empirical study of private synthetic data generation approaches.
    \item We propose a novel \textit{Direct Consistency Optimization} (DCO) approach which directly minimizes the difference between statistics of the original and the synthetic data. 
    \item We provide privacy guarantees for our DCO approach.
    \item We show that DCO works well when the data does not have complex structure. However, GAN-based approaches perform better in learning more complicated patterns in data.
\end{itemize}



\fi

\iffalse
\section{Private Training Algorithms}
\label{sec:privtrain}


The objective of a GAN is to solve the following min-max problem:
\begin{align*}
    \min_G \max_D \E_{x \sim p_X}[f(D(x))] + \E_{z \sim p_z} [f (1 - D(G(z)))].
\end{align*}
Here, $p_X$ denotes the data distribution and $p_z$ denotes a noise distribution; the function spaces for $G$ and $D$ are typically parameterized neural nets. The {\it measuring function} $f(x)$ is $\log(x)$ in the case of traditional GANs, corresponding to Jensen-Shannon divergence for the objective, and $x$ for Wasserstein GANs, corresponding to earth mover distance (which are our focus).
We are interested in training GANs subject to differential privacy.

\begin{definition}
A randomized algorithm $\mathcal{A} : \mathcal{X}^n \rightarrow \mathcal{R}$ with output domain $\mathcal{R}$ is $(\epsilon, \delta)$-differentially private (DP) if for all adjacent datasets $X, X' \in \mathcal{X}^n$ and for all $S \subseteq \mathcal{R}$: $P(\A(X) \in S) \leq e^{\epsilon} P(\A(X') \in S) + \delta$. 
\end{definition}

\subsection{Private Gradient Estimation}

GANs can be particulary sensitive to the choice of training algorithm, and in some cases we may be able to improve over differentially private Stochastic Gradient Descent by using a different update method.
In DPSGD, gradients for each sample are clipped before aggregating into a minibatch step, which is then perturbed with Gaussian noise. We consider a similar ``privatization'' of other commonly used algorithms such as Adam, Adagrad, RMSprop, and {\it optimistic} descent algorithms (the latter are discussed in \Cref{sec:optimistic}),
where we replace the gradient estimation step with that in \cite{Abadi_2016}.
We prove that each of these methods results in a GAN which satisfies differential privacy.

\begin{thm}\label{thm:privdescent}
Any training algorithm for the discriminator which computes a gradient estimate each round using clipping and Gaussian noise, and uses an arbitrary (possibly adaptively selected) combination of historical gradient estimates to make updates, satisfies the same privacy guarantee as DPSGD.
\end{thm}


\subsection{Optimistic Methods and Last-Iterate Convergence}
\label{sec:optimistic}
GANs are attempting to find an equilibrium of a zero-sum game. While many algorithms, including gradient descent, converge in zero-sum games when taking the average of action sequences (see e.g.\ \cite{cesabianchilugosi}), for GANs we typically aim to use a fixed network (often the final step), and so this theory does not apply even in the convex-concave setting
.
In \cite{daskalakis2017training}, {\it optimistic gradient descent} is shown to have last-iterate convergence when used in bilinear games, and is proposed as a method for training GANs for this reason. Extensive experimentation is also conducted with an optimistic variant of Adam, which they show often outperforms other methods.
%Further discussion of limit points of (optimistic) descent and ascent: \cite{daskalakis2018limit}.
In standard training via stochastic gradient descent, the two players update their weights as follows:
\begin{align*}
    w_{t+1} =&\; w_{t} + \eta \cdot \hat{\nabla}_{w,t} \\
    \theta_{t+1} =&\; \theta_{t} - \eta \cdot \hat{\nabla}_{\theta,t}
\end{align*}
Optimistic SGD uses the following update rule:
\begin{align*}
    w_{t+1} =&\; w_{t} + 2 \eta \cdot \hat{\nabla}_{w,t} -  \eta \cdot \hat{\nabla}_{w,t-1} \\
    \theta_{t+1} =&\; \theta_{t} - 2 \eta \cdot \hat{\nabla}_{w,t} +  \eta \cdot \hat{\nabla}_{w,t-1}
\end{align*}
Optimistic Adam replaces $\hat{\nabla}$ with the standard Adam update, and our private variants replace these gradient estimates with their clipped and perturbed analogues.

The theory of last-iterate convergence has been extended to handle stochastic updates and even to settings which are not convex-concave. If we have an {\it a priori} bound on the norm of the gradients during training, and the game satisfies  we can take Theorem 4.3 in \cite{mertikopoulos2018optimistic} to imply that Optimistic SGD with a decaying learning rate will converge to a saddle point, provided that that the function satisfies a property called {\it coherence}, which includes many non-convex-concave games.

Beyond goals of protecting sensitive data, private GANs also have benefits in preventing overfitting by memorization. 
A folklore theorem in the theory of differential privacy is that private learning algorithms cannot overfit, as a result of leave-one-out stability. The implication of this for training GANs is discussed in \cite{wu2019generalization}, but they do not conduct experiments involving private training. 
\fi





\iffalse

An alternate approach  for private synthetic data generation, given an original dataset $D \in. R^{d \times n}$ is to aim to approximately preserve a set of functions $\Ff$ on the dataset in hopes that these functions capture important features for downstream analysis (in the form of an explicit dataset rather than a list of queries). We show a method for achieving this, given access to an oracle for non-convex optimization. First we recall the Laplace mechanism from \cite{Dwork2006CalibratingNT}, a key ingredient in this approach. \wb{replace w Gaussian}




\subsection{The Laplace Mechanism}

The Laplace mechanism, introduced in \cite{Dwork2006CalibratingNT}, allows accurate private computation of statistics $f$ on a dataset when each $f$ is not too sensitive to changes in a single entry.

\begin{definition}[$\ell_1$-Sensitivity]
The $\ell_1$ sensitivity of a function $f: \N^{\abs{\X}} \rightarrow \R^k$ is: 
\begin{align*}
    \Delta f =&\; \max_{x, y \in \N^{\abs{\X}}, \norm{x-y}_1 = 1} \norm{f(x) - f(y)}_1.
\end{align*}
If we think of $f$ as a query to a dataset, this captures the maximum amount that the output of the query can change as a result of changing a single person's entry. 
\end{definition}
The extent to which we can accurately answer queries subject to differential privacy depends on the sensitivity of the queries we care about.
\iffalse
\begin{definition}[Laplace Distribution]
The Laplace Distribution (centered at 0) with scale parameter $b$ is the distribution with probability density function:
\begin{align*}
    \text{Lap}(x|b) =&\; \frac{1}{2b}\exp{(-\frac{\abs{x}}{b})}.
\end{align*}
The variance of this distribution is $\sigma^2 = 2b^2$ We can refer to a random variable sampled from this as $Y \sim \text{Lap}(b)$. If you've seen the exponential distribution before, this is a symmetric version of it.
\end{definition}
\fi

\begin{definition}[Laplace Mechanism]
Given any function $f: \N^{\abs{\X}} \rightarrow \R^k$, the Laplace mechanism is defined as:
\begin{align*}
    \M_L(x, f(\cdot), \epsilon) =&\; f(x) + (Y_1, \ldots, Y_k)
\end{align*}
where each $Y_i$ is drawn i.i.d from $\text{Lap}(\Delta f/\epsilon)$, with $\text{Lap}(x|b) = \frac{1}{2b}\exp{(-\frac{\abs{x}}{b})}$.
\end{definition}

\begin{theorem}[\cite{privacybook}]
The Laplace mechanism satisfies $\epsilon$-differential privacy.
\end{theorem}

\begin{theorem}[\cite{privacybook}] \label{thm:lap-acc}
Let $f: \N^{\abs{\X}} \rightarrow \R^k$, and let $y = \M_L(x, f(\cdot), \epsilon)$. Then for all $\delta \in (0,1]$:
\begin{align*}
    \Pr[\norm{f(x) - y}_{\infty} \geq \ln{\big(\frac{k}{\delta}\big)}\cdot \big(\frac{\Delta f}{\epsilon}\big)] \leq&\; \delta.
\end{align*}
\end{theorem}

\iffalse
\subsection{Creating Datasets Consistent with Many Queries}
Let $\Ff$ be a set of functions $f : \R^{d \times n} \rightarrow \R$, with $\abs{\Ff} = k$, with maximum sensitivity $\Delta f$. 
Let $\hat{\Ff} = \{ \hat{f}(D) | f \in \abs{\Ff} \}$ denote the set of function estimates computed by the Laplace mechanism on $d$. The objective for preserving answers to $f \in \Ff$ with a dataset $\D'$ in $\R^{d \times n'}$ is given by:
\begin{align}
    \min_{D' \in \R^{d \times n'}} \max_{f \in \Ff} \abs{\hat{f}(D) - f(D') } =&\; \min_{D' \in \R^{d \times n'}}  \norm{\hat{f}(D) - f(D') }_{\infty}. \label{eq:minmaxF}
\end{align}

If we can succeed in this optimization problem, 
\begin{theorem} \label{thm:dco-accuracy}
Let $n' = n$,  and let $\Delta f$ be the maximum sensitivity over $f \in \Ff$.
Suppose we have $D'$ which is a global minimizer for \cref{eq:minmaxF}. With probability at least $1 - \delta$, we have that $\max_{f \in \Ff} \abs{{f}(D) - f(D') } \leq 2 \ln(k / \delta) \cdot (\Delta f / \epsilon)$.
\end{theorem}
\begin{proof}
With probability $1 - \delta$, by \Cref{thm:lap-acc}, we have that 
$$\max_{f \in \Ff} \abs{\hat{f}(D) - f(D) } \leq \ln(k / \delta) \cdot (\Delta f / \epsilon).$$ By the existence of $D$, there must be some $D' \in \R^{d \times n}$ where $$\max_{f \in \Ff} \abs{\hat{f}(D) - f(D') } \leq \ln(k / \delta) \cdot (\Delta f / \epsilon),$$ as this holds when $D' = D$. Thus for any global minimizer $D'$, the theorem holds by the triangle inequality.
\end{proof}

Further, if the functions we care about are convex with respect to $D$, this optimization is tractable.
\begin{theorem} \label{thm:dco-alg}
If each $f \in \Ff$ is convex, and each row in $D$ has $\ell_2$ norm at most $C$, then there is an $\epsilon$-differentially private algorithm for finding a dataset $D'$ which preserves answers to each $f$ up to additive error $2 \ln(k / \delta) \cdot (\Delta f / \epsilon) + \alpha$, with probability $1 - \delta$, in time $\ppoly(n, d, C, 1/\alpha)$.
\end{theorem}
\begin{proof}
If each $f$ is convex, then so is the maximum in \cref{eq:minmaxF}, and the domain can be bounded as a function of $C$, allowing an $\alpha$-approximate solution to be found using standard convex optimization techniques. The error bound then follows from \Cref{thm:dco-accuracy}.
\end{proof}



In experiments, we additionally aim to preserve classes of functions which are non-convex, incl
This is hard in general, due to \cite{pcpsynthdatahard}, but we proceed using gradient descent. In particular, classes of queries we use for experiments are:
\begin{itemize}
    \item Column means: $f_i(D) = \frac{1}{n} \norm{\cdot D e_i}_1$, where $e_i$ is the $i$th standard basis vector of length $d$. 
    \item Column inner products: $f_{i,j} = \langle D e_i, D e_j \rangle $ 
    \item Column correlations: $f_{i,j} = \mSigma_{i,j}$, where $\mSigma$ is the covariance matrix of $D$ 
    \item Random projections: $[f] = D\cdot \rmW$, where $\rmW_{i,j} \sim U[-1, 1]$. 
\end{itemize}
We also consider as an objective
\begin{align*}
    \min_{D' \in \R^{d \times n'}}  \norm{\hat{f}(D) - f(D') }_p
\end{align*}
for values of $p$ other than $\infty$.
We use two different optimization methods for DCO: gradient descent directly on the objective, as well as simultaneous no-regret dynamics, similar to simultaneous descent as used for GANs.

\wb{discuss slack parameter}
\iffalse
\subsection{Direct Optimization on Violations}
If we can compute gradients for this objective with respect to the {\it entries} of $D'$, we can apply gradient descent directly to this objective \wb{which is not always convex...}.
With $p=\infty$, the set of solutions to this optimization problem is equivalent to the set of saddle points of the zero-sum game formulation.
\fi
\fi
\fi

==> prelims.tex <==
\section{Preliminaries}

\subsection{Additional Related Work}


Existing methods for generating private synthetic data generally fall into one of two categories. Some methods can generate datasets which are provably approximately consistent on large classes of queries, with modest data requirements, yet are computationally inefficient and often require exponential space.
{\it Can ``oracle-efficient'' methods in [CITE] be implemented without access to the exponential mechanism?}
Others can be specified to run in polynomial time, but do not come with provable guarantees and are primarily evaluated empirically. Private Generative Adversarial Networks (GANs) are a primary example of the latter... GANs  Wasserstein GANs are a popular variant wherein the discriminator learns the earth mover distance between distributions \cite{arjovsky2017wasserstein}.


%Problem: requiring oracle 
\wb{more in Quip doc, especially in unorganized links section}


\paragraph{Stability and Generalization in GANs}


\paragraph{Last-Iterate Convergence}



\paragraph{Private GANs}






How long do we need to train for? Limit cycles problem: if the model never converges, one may need to continually train and simultaneously generate samples in order to draw from the equilibrium (and this may not even approximate the equilibrium).
A common approach is to simply average the weights from many steps of training --- in theory, this only works for linear settings, but it appears to be somewhat effective in practice \cite{yazc2018unusual}. \wb{Similar kind of last-iterate guarantee for linear settings --- which works better in practice?}


For non-private GANs, the only cost in training longer than usual is computational, and we may be able to afford a lack of precision in specifying the exact. 

However, when privacy is a concern, we must me much more cautious in specifying the length to train for in order to stay within a privacy budget.
As such, we should be motivated to seek private methods for training GANs which converge to equilibrium more efficiently.

Training with Gaussian DP: \cite{bu2019deep} (not specific to GANs).
Mixed data types (Ankit's paper): \cite{tantipongpipat2019differentially}. Conditional GANs (generating labels): \cite{torkzadehmahani2020dpcgan}.





\paragraph{Privately Answering Many Queries}


\paragraph{Synthetic Data Release}

\subsection{Differential Privacy}


\begin{definition}[$(\epsilon,\delta)$-Differential Privacy]
A mechanism $\M$ is $(\epsilon,\delta)$-differentially private...
\end{definition}


\subsection{Wasserstein GANs}

Standard training via gradient descent:
\begin{align*}
    w_{t+1} =&\; w_{t} + \eta \cdot \nabla_{w,t} \\
    \theta_{t+1} =&\; \theta_{t} - \eta \cdot \nabla_{\theta,t} \\
\end{align*}

\input{privdescent}


\subsection{Optimistic Mirror Descent}

Training WGANs with Optimistic Mirror Descent:
\begin{align*}
    w_{t+1} =&\; w_{t} + 2\eta \cdot \nabla_{w,t} - \eta \cdot \nabla_{w,t-1} \\
    \theta_{t+1} =&\; \theta_{t} - 2\eta \cdot \nabla_{\theta,t} + \eta \cdot \nabla_{\theta,t-1}
\end{align*}
In the case of a zero-sum bilinear game given by a matrix $A$, this looks like: 
\begin{align*}
    x_{t} =&\; x_{t-1} - 2\eta Ay_{t-1} + \eta Ay_{t-2} \\
    y_{t} =&\; y_{t-1} + 2\eta A^T x_{t-1} - \eta \A^T x_{t-2}
\end{align*}

In \cite{daskalakis2017training}, it is shown in Theorem 1 that in this setting, $(x_t, y_t)$ approaches an equiilbrium as $t \rightarrow \infty$.

==> privdescent.tex <==
\subsection{Private Descent Methods}




\subsection{Private OMD}

\begin{algorithm} % enter the algorithm environment
\caption{Private Optimistic Mirror Descent} % give the algorithm a caption
\label{alg1} % and a label for \ref{} commands later in the document
\begin{algorithmic} % enter the algorithmic environment
\Input{}
\State  {\bf Initialize }$ \theta_0  \Leftarrow ...$
\For{$t \in [T]$}
    \State Take a random sample $L_t$
    \State {\bf Compute gradient}
    \State
    \State {\bf Clip gradient}
    \State 
    \State {\bf Descent}
    \State
\EndFor
\Output{}
\end{algorithmic}
\end{algorithm}





\begin{theorem}
... satisfies $(\epsilon, \delta)$-differential privacy ...
\end{theorem}

\subsubsection{Last-Iterate Convergence in Bilinear Games}


Does the last-iterate convergence result from \cite{daskalakis2017training} hold when gradient estimates are stochastic but unbiased? If this holds for appropriate noise distributions, then perhaps we can tell a story about last-iterate convergence in a toy GAN game which is linear but allows for a meaningful interpretation of privacy and subsampling for SGD.


I'm still parsing the proof of Theorem 1 in \cite{daskalakis2017training}. 
My intuition is that we'd have to very carefully define a distribution over gradient estimates for everything to go through --- we'd need several statements of equality in expected value to hold for iterated matrix products.
One idea is if each entry in $A$ is drawn independently for constructing updates $A^T x_t$ and $A y_t$.
But I'm not sure what the story about this would be.
If we think obtaining a theorem of this form would be a valuable part of a paper, I'd want to spend more time playing around with it to develop deeper intuition for what's going on. 



\subsection{Privacy Analysis}


==> proofs.tex <==
\subsection{Missing Proofs}

==> setup.tex <==
\subsection{Hyperparameters and Architectures}\label{architecture}
\begin{figure}[h]
\includegraphics[width=0.5\textwidth]{figs/diagram.png}
\caption{GAN Architecture for ADULT dataset experiments}
\end{figure}
